Time-Varying Convex Optimization via Time-Varying Averaged Operators

Devising efficient algorithms that track the optimizers of continuously varying convex optimization problems is key in many applications. A possible strategy is to sample the time-varying problem at constant rate and solve the resulting time-invariant problem. This can be too computationally burdensome in many scenarios. An alternative strategy is to set up an iterative algorithm that generates a sequence of approximate optimizers, which are refined every time a new sampled time-invariant problem is available by one iteration of the algorithm. These types of algorithms are called running. A major limitation of current running algorithms is their key assumption of strong convexity and strong smoothness of the time-varying convex function. In addition, constraints are only handled in simple cases. This limits the current capability for running algorithms to tackle relevant problems, such as $\ell_1$-regularized optimization programs. In this paper, these assumptions are lifted by leveraging averaged operator theory and a fairly comprehensive framework for time-varying convex optimization is presented. In doing so, new results characterizing the convergence of running versions of a number of widely used algorithms are derived.

==> my_sections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}


